Attention Driven Fusion for Multi-Modal Emotion Recognition

Deep learning has emerged as a powerful alternative to hand-crafted methods for emotion recognition on combined acoustic and text modalities. Baseline systems model emotion information in text and acoustic modes independently using Deep Convolutional Neural Networks (DCNN) and Recurrent Neural Networks (RNN), followed by applying attention, fusion, and classification. In this paper, we present a deep learning-based approach to exploit and fuse text and acoustic data for emotion classification. We utilize a SincNet layer, based on parameterized sinc functions with band-pass filters, to extract acoustic features from raw audio followed by a DCNN. This approach learns filter banks tuned for emotion recognition and provides more effective features compared to directly applying convolutions over the raw speech signal. For text processing, we use two branches (a DCNN and a Bi-direction RNN followed by a DCNN) in parallel where cross attention is introduced to infer the N-gram level correlations on hidden representations received from the Bi-RNN. Following existing state-of-the-art, we evaluate the performance of the proposed system on the IEMOCAP dataset. Experimental results indicate that the proposed system outperforms existing methods, achieving 3.5% improvement in weighted accuracy.

==> results.tex <==
\section{Experiments}

\subsection{Dataset and Experimental Setup}

Experiments are conducted on the Interactive Emotional Dyadic Motion Capture (IEMOCAP) dataset which includes five sessions of utterances for 10 unique speakers. We follow the evaluation protocol of \cite{yoon2019speech, yoon2018multimodal}, and select utterances annotated with four basic emotions \enquote{anger}, \enquote{happiness}, \enquote{neutral} and \enquote{sadness}. Samples with \enquote{excitement} are merged with \enquote{happiness} as per \cite{yoon2019speech, yoon2018multimodal}. The resultant dataset contains $5531$ utterances \{\enquote{anger}:$1103$, \enquote{happiness}:$1636$, \enquote{neutral}:$1708$, \enquote{sadness}:$1084$\}. 

Initial training is carried out on both acoustic and textual networks separately before the fusion. The sampling rate of each utterance waveform is set to $16,000$Hz while a random segment of $250ms$ is used in training the acoustic network. During the evaluation, the cumulative sum of all the predictions with a window size and shift of $250ms$ and $10ms$ are considered. In the textual network, all the transcripts of the utterances are set to a maximum length of $100$ and padded with 0s. Glove-300d embeddings are used to convert the word sequence to a vector of $(100,300)$. \textcolor{black}{We utilize a 10-fold cross-validation with an 8:1:1 split for training, validation, and test sets respectively for text model. We select an average performing split and use this split to train the acoustic and fusion networks (we use a single split due to the high computation time of the acoustic model), such that all networks (text, audio and fusion) use the same data splits.} The learning rate and the batch size in each network are fixed at $0.001$ and $64$ respectively, and the Adam optimiser is used. 

\subsection{Performance Evaluation and Analysis}

Following \cite{yoon2019speech, yoon2018multimodal}, the performance of our system is measured in terms of weighted accuracy (WA) and unweighted accuracy (UA). Table \ref{acc} and Figure \ref{fig:confusion} present performance of our approach for emotion recognition compared with the state of the art methods.

\begin{figure*}
\centering
%\includegraphics[width=16.5cm, height=9cm]{./figures/nnb.png}
\includesvg[width=17.5cm]{./confusion.svg}
\caption{Confusion matrices of the proposed architecture for separate fusion methods calculated using a average performing 8:1:1 split. Left, middle and right figures represent Fusion I, Fusion II and Fusion III respectively.}
\label{fig:confusion}
\vspace{-2mm}
\end{figure*}

MDRE \cite{yoon2018multimodal} has used two RNNs to encode both acoustic and textual data followed by a DNN for classification, while Evec-MCNN-LSTM \cite{cho2018deep} has used an RNN and a DCNN to encode both modalities followed by fusion and an SVM for classification. MHA-2 \cite{yoon2019speech} has used two Bidirectional Recurrent Encoders (BRE) for both modalities followed by a multi-hop attention mechanism. MDRE has outperformed MCNN-LSTM by $10.6\%$ and MHA-2 has outperformed MDRE by $6.5\%$, demonstrating how attention can increase performance.

Our proposed model has achieved a substantial improvement in overall accuracy, with a $3.5\%$ increase compared to MHA-2. We have utilized self-attention before (F-III) and after fusion (F-II) as illustrated in Figure \ref{fig:nn}. Cross-modal attention has not been utilized after fusion since the dimensionality of the feature vectors from the two modalities are different. A slight increase in the classification accuracy has been obtained by applying self-attention compared to conventional feature fusion (F-I). Furthermore, the highest accuracy has been obtained by \textbf{F-III}, outperforming F-II by $0.5\%$. Given that F-I slightly outperforms MHA-2, we have compared the classification accuracy of the individual modes of MHA-2 with our individual modes in Table \ref{acci}.

\begin{table}[t]
\centering
\begin{tabular}{|c|c|c|c|c|} 
\hline 
Model & Modality & WA & UA \\ [0.5ex]
\hline \hline
Evec-MCNN-LSTM \cite{cho2018deep}& $A+T$ & $64.9\%$ & $65.9\%$\\
MDRE \cite{yoon2018multimodal}& $A+T$ & $71.8\%$ & $-$\\
MHA-2 \cite{yoon2019speech}& $A+T$ & $76.5\%$ & $77.6\%$\\
\hline
\textbf{Ours - F-I} & $A+T$ & $\textcolor{black}{77.85\%}$ & $\textcolor{black}{79.27\%}$\\
\textbf{Ours - F-II} & $A+T$ & $\textcolor{black}{78.98\%}$ & $\textcolor{black}{80.01\%}$\\
\textbf{Ours - F-III} & $A+T$ & $\textcolor{black}{\textbf{79.22\%}}$ &$\textcolor{black}{\textbf{80.51\%}}$\\
\hline
\end{tabular}
\caption{\textcolor{black}{Recognition accuracy for IEMOCAP using an average performing 8:1:1 split, compared with state of the art methods.}}

\label{acc}
\end{table}

\begin{table}[t]
\centering
\begin{tabular}{|c|c|c|} 
\hline 
Model & Modality & WA \\ [0.5ex]
\hline \hline
MHA-2 \cite{yoon2019speech}& $A$  & $65.2\%$\\
MHA-2 \cite{yoon2019speech}& $T$  & $70.3\%$\\
\hline
\textbf{Ours} & $A$  & \textcolor{black}{$\textbf{69.8\%}$}\\
\textbf{Ours} & $T$  & \textcolor{black}{$\textbf{67.3\%}$}\\
\hline
\end{tabular}
\caption{\textcolor{black}{Recognition accuracy of individual modes of the IEMOCAP dataset with an average performing 8:1:1 split, comparing the proposed approach with \cite{yoon2019speech}.}}
\label{acci}
\end{table}

Our acoustic and textual models outperformed the corresponding individual modes of MHA-2 \cite{yoon2019speech}, where a substantial improvement of $\textbf{7.2\%}$ is achieved with the acoustic model. The SincNet layer in the acoustic model is capable of learning and deriving customized filter banks tuned for emotion recognition. It has been successfully applied for speaker recognition \cite{ravanelli2018speaker} as an alternative to i-vectors. The confusion matrices for F-I, F-II, and F-III are illustrated in Figure \ref{fig:confusion}. A $\textbf{10.6\%}$ relative improvement in classification accuracy can be observed when comparing the individual modalities with the fusion network in our model. Given that accuracy is approximately similar for both modalities, each modality has complemented the other to increase recognition accuracy. 

\vspace{-5mm}


